Visual Attention driven by Convolutional Features

The understanding of where humans look in a scene is a problem of great interest in visual perception and computer vision. When eye-tracking devices are not a viable option, models of human attention can be used to predict fixations. In this paper we give two contribution. First, we show a model of visual attention that is simply based on deep convolutional neural networks trained for object classification tasks. A method for visualizing saliency maps is defined which is evaluated in a saliency prediction task. Second, we integrate the information of these maps with a bottom-up differential model of eye-movements to simulate visual attention scanpaths. Results on saliency prediction and scores of similarity with human scanpaths demonstrate the effectiveness of this model.

==> section2_themodel.tex <==
\section{Variational Laws of Visual Attention}
Regardless of the implementation that evolution has developed, the visual attention mechanisms aim to satisfy the needs of visual information in foveated animals. Therefore, evolution was guided by this functional principle. In this work, we have tried to derive differential laws that describe the natural implementation of just three basic principles. These principles are presented in the following subsection. Subsequently, the laws of attention are derived mathematically on the basis of the principle of least action in physics.

\subsection{Principles of visual attention}
The \textit{brightness} signal $b(t, x)$ can be thought of as a real-valued function
		\begin{equation}
			b:\R^+ \times \R^2 \to \R
		\end{equation}
where   $t$ is the time and $x=(x_1, x_2)$ denotes the position.
The {\em scanpath} over the visual input is defined as
		\begin{equation}
			x: \R^+  &\to \R^2 
		\end{equation}
The scanpath $x(t)$ will be  also referred to  as \textit{trajectory} or \textit{observation}.

Three fundamental principles drive the model of attention. They lead to the 
introduction of the correspondent terms of the Lagrangian of the action.
\begin{enumerate}
\item [i)] {\em Boundedness of the trajectory} \\
	Trajectory $x(t)$ is bounded into a defined area (retina). 
	This is modeled by a harmonic oscillator at the borders of the image
	which constraints the motion within the retina\footnote{Here, we use
	Iverson's notation, according to which if $p$ is a proposition then
	 $[p]=1$ if $p$={\tt true} and $[p]=0$ otherwise}:
	\begin{equation} \label{retina}
	V(x) = k \sum_{i=1,2} \big( \left( l_i - x_i\right)^2 \cdot \left[ x_i > l_i \right] + \left( x_i \right)^2 \cdot \left[ x_i < 0 \right] \big)
	\end{equation}
	where $k$ is the elastic constant, $l_i$ is the i-th dimension of the rectangle
	which represents the retina\footnote{A straightforward extension can be 
	given for circular retina.}. 
	
\item [ii)] \textit{Curiosity driven principle} \\
	Visual attention is attracted by regions with many details, that is where
	the magnitude of the gradient of the brightness is high. In addition to this 
	local field, the role of peripheral information is included 
	by processing a blurred version $p(t,x)$ of the brightness $b(t,x)$. 
	The modulation of these two terms is given by
	\begin{equation}\label{curiosity}
 		C(t, x) =  b_x^2 \cos^2(\omega t) 
		+ p_x^2 \sin^2(\omega t), 
	\end{equation}
	where $b_x$ and $p_x$ denote the gradient w.r.t.\@ $x$.
	Notice that the alternation of the local and peripheral fields 
	has a fundamental role in avoiding trapping into regions with
	too many details.	
	
\item [iii)] \textit{brightness invariance} \\
	Trajectories that exhibit \textit{brightness invariance} are
	 motivated by the need to perform fixation. 
	Formally,  we  impose the constraint
	$\dot{b} = b_t + b_{x} \dot{x} = 0$.
	This is in fact the classic constraint that is widely used in computer vision
	for the estimation of the optical flow~\cite{optflow}. Its soft-satisfaction can 
	be expressed by the associated term
	\begin{equation}\label{bi}
		B(t,x, \dot x) = \big(b_t + b_{x} \dot{x}\big)^{2}.
	\end{equation}
	Notice that, in the case of static images, $b_t = 0$, and the term is fully satisfied for trajectory $x(t)$ whose velocity $\dot x$ is perpendicular to the gradient, 
	\ie when the focus is on the borders of the objects. 
	This kind of behavior favors coherent fixation of objects. 
	Interestingly, in case of static images, the model can conveniently be simplified by 
	using the upper bound of the brightness as follows:
	\begin{align}\label{Bbar}
	\begin{split}
	B(t,x,\dot x) & = \dot{b}^{2}(t,x) = (\partial b_{t} + b_{x} \dot{x})^{2} \le \\
	& \le 2 b_{t}^2 + 2 b_{x}^2  \dot{x}^{2}:= \bar B(t, x, \dot x)
	\end{split}
	\end{align}
    This inequality comes from the parallelogram law of Hilbert spaces. 
    As it will be seen the rest of the paper, this approximation significantly simplifies the
    motion equations.
\end{enumerate}
    \subsection{Least Action Principle}
    Visual attention scanpaths are modeled as the motion of a particle of mass $m$ within a potential field. This makes it possible to construct the generalized action
		\begin{equation} \label{S}
		S = \int^T_0 L(t, x, \dot x) \,dt
		\end{equation}
		where $L=K-U$,  where $K$ is the kinetic energy
		\begin{equation} \label{K}
		K(\dot x)= \frac{1}{2}m \dot{x}^2
		\end{equation}
		and $U$ is a generalized potential energy defined as 
		\begin{equation} \label{U}
		U(t, x, \dot x) = V(x) - \eta C(t, x) + \lambda B(t, x, \dot x).
		\end{equation}
		Here, we assume that $\eta,\lambda >0$. Notice, in passing
		that while $V$ and $B$ get the usual sign of potentials, $C$ comes with the flipped
		sign. This is due to the fact that, whenever it is large, it generates an attractive field. 
		In addition, we notice that the brightness invariance term is not a truly potential,
		since it depends on both the position and the velocity. However, its generalized interpretation as a ``potential'' comes from
		considering that it generates a force field. 
		In order to discover the trajectory we look for a stationary point 
		of the action in Eq.~\eqref{S}, which corresponds to the Euler-Lagrange 
		equations
		\begin{equation}\label{ELeq_}
		\dfrac{d}{dt} \dfrac{\partial L}{\partial \dot x_i} = \dfrac{\partial L}{\partial x_i}, 
		\end{equation} 
		where $i=1,2$ for the two motion coordinates. 		
		The right-hand term in \eqref{ELeq_} can be written as
		\begin{equation}\label{dLdx}
		\dfrac{\partial L}{\partial x} = \eta C_{x} - V_{x}- \lambda 
		B_{x} .
		\end{equation}
		Likewise we have 
		\begin{equation}\label{dLddotx}
		\dfrac{d}{dt} \dfrac{\partial L}{\partial \dot x}  = m \ddot{x}- \lambda  \frac{d}{dt} B_{\dot{x}}
		\end{equation}
		so as the general motion equation turns out to be 
		\begin{equation}\label{equations_of_motion_general_form}
		m \ddot{x}- \lambda  \frac{d}{dt} B_{\dot{x}} +
		V_{x} - \eta C_{x} + \lambda 
		B_{x}  = 0.
		\end{equation}
		These are the general equations of visual attention. 
		In the Appendix we give the technical details
		of the derivations. Throughout the paper, the proposed
		model is referred to as the EYe MOvement Laws (EYMOL).
		
	\subsection{Experimental results on saliency prediction}
	
	Discussion over experimental setup and results from nips 2017 goes here
	
	
    \begin{table*}[h]
	\begin{center}
		\begin{tabular}{|l|c c c c c c|}
			\hline
			& \multicolumn{6}{|c|}{CAT2000-TEST}\\
			& AUC & SIM & EMD & CC & NSS & KL\\
			\hline\hline			
			{\small Itti-Koch~\cite{itti1998}, implem. by~\cite{harel}} & 0.77 & 0.48 & 3.44  & 0.42 & 1.06 & \textbf{0.92} \\
			\hline			
			{\small AIM~\cite{aim}}  & 0.76 & 0.44 & 3.69 &  0.36 & 0.89 & 1.13 \\
			\hline		
			{\small Judd Model~\cite{Judd} } & 0.84 & 0.46 & 3.60 & 0.54 & 1.30 & 0.94\\
			\hline			
			{\small AWS~\cite{aws}} & 0.76 & 0.49 & 3.36  & 0.42 & 1.09 & 0.94\\
			\hline
			{\small eDN~\cite{eDN}} & \textbf{0.85} & 0.52 & 2.64  & 0.54 & 1.30 & 0.97\\
			\hline
			{\small \textbf{EYMOL}} & 0.83 &\textbf{ 0.61} & \textbf{1.91} & \textbf{0.72} & \textbf{1.78} & 1.67\\	
			\hline				
		\end{tabular}
	\end{center}
	\vspace{-0.5em}
	\caption{Results on CAT2000~\cite{cat2000} provided by MIT Saliency Benchmark Team \cite{mit-saliency-benchmark}. The models are sorted chronologically. In bold, the best results for each metric and benchmarks.}\label{tab:scorecat}
	\end{table*}	
		
